Offline Reinforcement Learning via Linear-Programming with Error-Bound Induced Constraints

Offline reinforcement learning (RL) aims to find an optimal policy for Markov decision processes (MDPs) using a pre-collected dataset. In this work, we revisit the linear programming (LP) reformulation of Markov decision processes for offline RL, with the goal of developing algorithms with optimal $O(1/\sqrt{n})$ sample complexity, where $n$ is the sample size, under partial data coverage and general function approximation, and with favorable computational tractability. To this end, we derive new \emph{error bounds} for both the dual and primal-dual formulations of the LP, and incorporate them properly as \emph{constraints} in the LP reformulation. We then show that under a completeness-type assumption, $O(1/\sqrt{n})$ sample complexity can be achieved under standard single-policy coverage assumption, when one properly \emph{relaxes} the occupancy validity constraint in the LP. This framework can readily handle both infinite-horizon discounted and average-reward MDPs, in both general function approximation and tabular cases. The instantiation to the tabular case achieves either state-of-the-art or the first sample complexities of offline RL in these settings. To further remove any completeness-type assumption, we then introduce a proper \emph{lower-bound constraint} in the LP, and a variant of the standard single-policy coverage assumption. Such an algorithm leads to a $O(1/\sqrt{n})$ sample complexity with dependence on the \emph{value-function gap}, with only realizability assumptions. Our properly constrained LP framework advances the existing results in several aspects, in relaxing certain assumptions and achieving the optimal $O(1/\sqrt{n})$ sample complexity, with simple analyses. We hope our results bring new insights into the use of LP formulations and the equivalent primal-dual minimax optimization for offline RL, through the error-bound induced constraints.

==> Best_Covered.tex <==
\subsection{Extension: Best Covered Policy}

Our proof can be readily  adapted to the case where the function class does not cover the optimal $w^*$, and the optimal policy is not well-covered by the data (with almost the same proof). We provide the proofs as below. 

\subsubsection{Case 1.} 
We first introduce the same definition of $C$-covered policy as in [Zhan et al., 2022]. 

\begin{Definition}[$C$-covered policy.]  
We say a policy $\pi$ is $C$-covered by the data if 
$$\theta_{\pi}(s,a)\le C\cdot \mu(s,a),~~\forall s,a.$$ Further, we say $\pi^*_C$ is an \emph{optimal $C$-covered policy} if it maximizes $J(\pi)$ among all $C$-covered policies. 
\end{Definition}


We assume the realizability of the optimal $C$-covered policy in the following assumption:

\noindent\textbf{Assumption 1.}
There exists a $\bar{w}\in W$ such that $\bar{w}(s,a)=\theta_{\pi^*_C}(s,a)/\mu(s,a)$ for some optimal $C$-covered policy $\pi^*_C$. 

Note that here we do not assume realizability of the $w^*$, but only that of $\bar{w}$, since we are not aiming for finding the optimal policy, but just the best covered policy. 

By the definition and assumption above, we know   the following optimization problem is feasible:  
\begin{align} 
&\min_{w\in W}~~~~(-u^\top w)\\
&s.t.~~~~~~Kw=(1-\gamma)\mu_0,~~\|w\|_\infty\le C.
\end{align} 
Let $w_W^*$ denote the optimal solution to this problem.  


Then, we solve the following empirical version of the problem  to obtain $w_{\mathcal{D}}$:
\begin{align}
&\min_{w\in W}~~~~(-u_{\mathcal{D}}^\top w)\\
&\text{s.t.}~~~~ x^\top(K_{\mathcal{D}}w-(1-\gamma)\mu_0)\le E_{\delta,n,W},\forall x\in B\\
&~~~~~~\|w\|_{\infty}\le C,
\end{align}
where $E_{\delta,n,W}=C\sqrt{2\log(|B||W|/\delta)}/\sqrt{n}$. 
Let $\pi_{\mathcal{D}}=\pi_{w_{\mathcal{D}}}$.  Then we have the following theorem:
 
\begin{Theorem}
With probability at least $1-\delta$, we have
$$J(\pi_C^*)-J(\pi_{\mathcal{D}})\le \tilde{O}\big({C\sqrt{\log(|B||W|/\delta)}}/((1-\gamma)\sqrt{n})\big).$$
\end{Theorem}

The proof is similar to that of the main results in \S\ref{sec:func_1}  (c.f. Theorem \ref{main1} and Theorem \ref{tabular_main}). 
First, we prove the feasibility of $w_W^*$ to this empirical problem by using concentration bound and union bound for all $x$ in $B$. 
Next, using the feasibility and concentration bound, we have
$$u^\top w_{\mathcal{D}}\ge u^\top w_W^*+\tilde{O}(1/\sqrt{n}).$$
Next, using the error bound result  (Lemma \ref{lemma:infeasible}), we have $|J(\pi_{\mathcal{D}})-u^\top w_{\mathcal{D}}|\le \|Kw_{\mathcal{D}}-(1-\gamma)\mu_0\|_1/(1-\gamma)$.
Combining the above, we have the desired result.
\subsubsection{Case 2.}
For convenience, we also assume that the optimal policy is unique as in [Chen and Jiang, 2022]. We also need the definition of (optimal) $C$-covered policy as above in \textbf{Case 1}, but with the $\theta_\pi$ therein being replaced by $\theta_{\pi,\mu}$.  Note that such a slight difference also mirrors that in the SPC assumptions used in \S\ref{sec:func_1} and \S\ref{sec:second_FA}. We will only consider this $\mu$-dependent assumptions and definitions in this \textbf{Case 2}, and omit the $\mu$-dependence for notational simplicity.  

Then we make the following SPC assumption, which is similar to Assumption \ref{SPC}:

\begin{Assumption} \label{assum:add_best_cover}
There exists a $\bar{w}\in W$ such that $\bar{w}(s,a)=\theta_{\pi^*_C}(s,a)/\mu(s,a)$ for some optimal $C$-covered policy $\pi^*_C$. 
\end{Assumption}

Following our algorithm in \S\ref{sec:second_FA}, we consider the following minimax problem: 
\begin{align}
&\min_{w\in W}\max_{v\in V}~~~~(-u^\top w+v^\top(Kw-(1-\gamma)\mu))\\
&~~~\mathrm{s.t.}~~~~~~~\|w\|_{\infty}\le C,~~ \sum_aw(s,a)\pi_{\mu}(a\mid s)\ge 1-\gamma. 
\end{align}
We denote the optimal solution of the above problem as $w_W^*$. Then,  
we obtain $w_{\mathcal{D}}$ by solving the following empirical version of the problem, and denote its optimal solution as $w_{\mathcal{D}}$:
\begin{align}
&\min_{w\in W}\max_{v\in V}~~~~~~(-u_{\mathcal{D}}^\top w+v^\top(K_{\mathcal{D}}w-(1-\gamma)\mu_{\mathcal{D}}))\\
&\mathrm{s.t.}~~~~\|w\|_{\infty}\le C,~~ \sum_aw(s,a)\pi_{\mu}(a\mid s)\ge 1-\gamma.
\end{align}

For simplicity, we assume that $v^*\in V$. Then we additionally make the following assumption regarding the sub-optimality of the $C$-covered policy:

\begin{Assumption}\label{assum:context_bandit_sub_opt}
We assume that $w_W^*$ satisfies that 
$$
\sum_{s\in S}\Bigg|\sum_{a\in A}\big(w_W^*(s,a)-w^*(s,a)\big)\Bigg|\le \epsilon
$$ for the  optimal $w^*$. 
\end{Assumption}
 
This assumption characterizes how far away the optimal solution of the optimization problem above, $w_W^*$, is from $w^*$. This immediately  leads to the following result: 
\begin{equation}\label{equ:sum}
	\sum_{s\in S}\Bigg|\sum_{a\in A}\big(w_W^*(s,a)-w^*(s,a)\big)\pi_\mu(a\mid s)\Bigg|\le \epsilon. 
\end{equation}

 Under this Assumption \ref{assum:context_bandit_sub_opt}, we can directly compare $w_{\mathcal{D}}$ to the optimal $w^*$, and the resulting bound has an additional term depending on $\epsilon$. 

Concretely speaking, we have the following theorem:

\begin{Theorem}
With probability at least $1-\delta$,
$$J(\pi^*)-J(\pi_{\mathcal{D}})\le 
\frac{1}{(1-\gamma)^3}\cdot \Big(\frac{{4\sqrt{2}C}\sqrt{\log(|V||W|/\delta)}}{\Delta_Q\sqrt{n}}+\frac{2\epsilon}{\Delta_Q}\Big)\cdot (C+\epsilon).$$
\end{Theorem}

Since $\|u\|_{\infty}\le 1$ (where we recall $u(s,a)=r(s,a)\cdot \mu(s,a)$) and $\|v\|_\infty\le 1/(1-\gamma)$, we can easily prove that $\ell(w)$ is $\big(2/(1-\gamma)\big)$-Lipschitz with respect to $L_1$-norm. 
Therefore, $\ell(w_W^*)-\ell(w^*)\le 2\epsilon/(1-\gamma)$.

Using the same argument as the proofs in \S\ref{sec:second_FA}, we have $\ell(w_{\mathcal{D}})-\ell(w_W^*)\le \frac{{4\sqrt{2}C}\sqrt{\log(|V||W|/\delta)}}{(1-\gamma)\sqrt{n}}$. 
Therefore,  we have that the population primal gap  $\Delta(w_{\mathcal{D}})\le \frac{{4\sqrt{2}C}\sqrt{\log(|V||W|/\delta)}}{(1-\gamma)\sqrt{n}}+\frac{2\epsilon}{1-\gamma}$. Then by Lemma \ref{inactive}, we have 
$$E_I:=\sum_{(s,a)\in \mathcal{I}}w_{\mathcal{D}}(s,a)\mu(s,a)\le \frac{\Delta(w_{\mathcal{D}})}{\Delta_Q}.$$

Then also following the arguments before, we have the following bound, which is similar to the derivations around Eq. \eqref{key+}:
\begin{align}
&J(\pi^*)-J(\pi_{\mathcal{D}})\\
&\le \frac{2E_I}{1-\gamma}\cdot \max_{s\in S}(\frac{\theta_{\pi^*}(s)/\mu(s)}{\sum_aw_{\mathcal{D}}(s,a)\pi_{\mu}(a\mid s)})\\
&\le\frac{2E_I}{1-\gamma}\max_{s\in S}\frac{\theta_{\pi_w^*}(s)/\mu(s)}{1-\gamma}+2\epsilon E_I/(1-\gamma)^2,\\
&\le 2CE_I/(1-\gamma)^2+2\epsilon E_I/(1-\gamma)^2,
\end{align}
where the second inequality uses Eq. \eqref{equ:sum} and the lower bound constraints of $\sum_aw(s,a)\pi_{\mu}(a\mid s)$, and the last inequality is because of \textbf{Assumption 2}. 
Hence, we have the desired result.

==> Contextual_Bandit.tex <==
\subsection{Extension: Contextual Bandit without Completeness}

We now consider a simplified setting than that introduced in \S\ref{sec:background},  i.e., the contextual bandit setting, where there state is drawn from a fixed distribution. We show below that our  results can be specialized to this case without completeness assumption (c.f. Assumption \ref{ass:f1_fake} in \S\ref{sec:func_1}).  
 
%\subsubsection{Contextual Bandit Setup}

%\kz{formally introduce the CB setup.}

\subsubsection{Results}
As stated in \S\ref{sec:background}, contextual bandit is a special case of learning in discounted MDP with $\gamma=0$.
We now introduce the LP for the contextual-bandit case: 
\begin{align}
&\min_{w\ge 0}~~~~(-u^\top w)\\
&\text{s.t.}~~~~~~\Omega w=\mu_0, w\in W,
\end{align}
where $\Omega=\mathrm{diag}(\Omega_1,\cdots,\Omega_{|S|})$ with $\Omega_i=(\mu(s^i,a^1),\cdots,\mu(s^i,a^{|S|}))$.
We use function approximation to $w$ and $\mu$ here, i.e., $w\in W$ and $\mu\in U$ for some function classes $W$ and $U$. First, we use $\hat{\mu}_{D}$ to estimate $\mu$  by maximum likelihood estimation (MLE):
$$\hat{\mu}_{\mathcal{D}}=\arg\max_{\mu'\in U}~~E_{(s,a)\sim \mu_{\mathcal{D}}}\log \mu'(s,a).$$
With this MLE estimator, the algorithm still falls into our LP framework, though it is slightly different from that for the MDP case. Note that even in [Rashidinejad et al., 2022], the algorithms for the contextual-bandit and MDP cases are different. 





By standard MLE convergence  results (see e.g., [Van de Geer, 2000, Chapter 7], or [Agarwal et al., 2020, Theorem 21]), we have  the following lemma:

\begin{Lemma}\label{mle}
With probability $\ge 1-\delta$, we have
$$\|\hat{\mu}_{\mathcal{D}}-\mu\|_1\le O(\sqrt{\log (|U|/\delta)}/\sqrt{n}).$$
\end{Lemma}
We next solve the following empirical problem for the contextual-bandit case:
\begin{align}
&\min_{w\ge 0}~~~~(-u_{\mathcal{D}}^\top w)\\
&\text{s.t.}~~~~~~\|\Omega_{\mathcal{D}} w-\mu_0\|_1\le E_{\delta,n}, w\in W,
\end{align}
where $E_{\delta,n}=6\sqrt{\log(|U|/\delta)}/\sqrt{n}$ and $\Omega_{\mathcal{D}}=\mathrm{diag}(\Omega_{1,D},\cdots, \Omega_{|S|,D})$ with 
$$
\Omega_{i,D}=(\hat{\mu}_{\mathcal{D}}(s^i,a^1),\cdots, \hat \mu_{D}(s^i,a^{|S|})).
$$ 

This Lemma \ref{mle} plays the same role as Eq. \eqref{single_concentration}, in the contextual-bandit case. This lemma is used to prove that $w^*$ is feasible with high probability. 
Then using similar arguments   that proved Theorem \ref{main1} (importantly Lemma \ref{lemma:infeasible} in the paper), we have
\begin{Theorem}
With probability $\geq 1-\delta$, we have 
$$J(\pi^*)-J(\pi_{\mathcal{D}})\le \tilde{O}(\sqrt{\log(|W||U|/\delta)}/\sqrt{n}).$$
\end{Theorem}

\paragraph{Remark.}
Notice that in contextual bandits, we do not need to deal with the transition matrix. Also, we propose to approximate $\mu$ in the algorithm. In this case, we do not need to use the sign function $x$ to deal with the $\ell_1$ norm violation of the constraint, and thus do not need the completeness of the corresponding function class $B$. 
Moreover, when $n$ is sufficiently large, say, $n\ge \Omega(|A|)$, we do not need to approximate $\mu$. This can be proved similar to that in \S\ref{sec:armdp}.
